Applications of Deep Learning for Top-View Omnidirectional Imaging: A Survey

A large field-of-view fisheye camera allows for capturing a large area with minimal numbers of cameras when they are mounted on a high position facing downwards. This top-view omnidirectional setup greatly reduces the work and cost for deployment compared to traditional solutions with multiple perspective cameras. In recent years, deep learning has been widely employed for vision related tasks, including for such omnidirectional settings. In this survey, we look at the application of deep learning in combination with omnidirectional top-view cameras, including the available datasets, human and object detection, human pose estimation, activity recognition and other miscellaneous applications.

==> sec/architecture.tex <==
\section{Network architecture}
\label{sec:architecture}

In previous sections, most authors use CNNs that are developed for perspective images.
Either by projecting the omnidirectional image into normal perspective, or with additional data, these CNNs are able to perform object detection, pose estimation and various other tasks in omnidirectional images.
However, there is another possibility to solve the problem.
Researchers try to adapt the network architecture specifically for omnidirectional images.
Although not directly designed for the top-view, these networks have been applied to other types of omnidirectional or spherical images \textbf{\MakeUppercase{citations here needed}}, thus we present them to show this possibility.

Spherical CNNs \cite{cohen2018sphericalcnns} and SphereNet\cite{coors2018spherenet} are two pioneers in network architecture to address the spherical image space.
For \textbf{spherical CNNs}, the translational movement of filters in 2D space \(\mathbb{Z}^2\) corresponds to the rotational movement in the 3D spherical space \(SO(3)\).
To calculate the spherical correlation efficiently (the term used by the authors, which can be understood as the convolution in normal CNNs), the authors implemented generalized fast Fourier transformation (GFFT).
The implementation with PyTorch is available at \url{https://github.com/jonkhler/s2cnn}.
Test results on the spherical MNIST dataset and the SHREC17 task \cite{savva2017large} show the robustness of the presented implementation.
\textbf{SphereNet} projects the filters of regular CNNs on the tangent plane of the sphere, thus gaining the ability to adapt existing CNNs for equidistant representations.
Unlike spherical CNNs, which are fully invariant for 360°, SphereNet is only invariant to the latitudinal rotations.
Its ability to make use of existing CNN architectures enables it to perform different computer vision tasks such as classification and object detection using transfer learning.

Since we are only presenting these research works as a future direction for top-view omnidirectional images, we don't get deeper in this topic. Interested readers can find further developments of this areas in publications such as \cite{perraudin2019deepsphere,jiang2019spherical,su2019kernel,lee2019spherephd,cohen2019general,ao2021spinnet}.

==> sec/depth.tex <==
\section{Depth estimation}
\label{sec:depth}
